$\textit{sweet}$- An Open Source Modular Platform for Contactless Hand Vascular Biometric Experiments

Current finger-vein or palm-vein recognition systems usually require direct contact of the subject with the apparatus. This can be problematic in environments where hygiene is of primary importance. In this work we present a contactless vascular biometrics sensor platform named \sweet which can be used for hand vascular biometrics studies (wrist, palm, and finger-vein) and surface features such as palmprint. It supports several acquisition modalities such as multi-spectral Near-Infrared (NIR), RGB-color, Stereo Vision (SV) and Photometric Stereo (PS). Using this platform we collect a dataset consisting of the fingers, palm and wrist vascular data of 120 subjects and develop a powerful 3D pipeline for the pre-processing of this data. We then present biometric experimental results, focusing on Finger-Vein Recognition (FVR). Finally, we discuss fusion of multiple modalities, such palm-vein combined with palm-print biometrics. The acquisition software, parts of the hardware design, the new FV dataset, as well as source-code for our experiments are publicly available for research purposes.

==> per_finger_fvr_table.tex <==
%!TeX root=main.tex

% this table is correct
\begin{table*}
\caption{\small \tred{fix caption. Check dev-fmr for all three fingers.} Index-Finger-vein recognition performance at FMR no greater than 0.1\% on the Dev set.
%HTER is the average of the FMR and FNMR in each row.
%The FMR, FNMR and HTER values in the table indicate percentages.
%The score-threshold has been computed to achieve the desired FMR (0.1\%) on the Dev set.
%This score-threshold has then been applied to the comparison-scores obtained from the Eval set.
The lowest HTER for this finger is marked in bold characters, and comes from RH\_left\_950 protocol.
}
\ra{1.1}
\center
\small
\vspace{-2mm}
\begin{tabular}{p{4.5mm}|p{3.8mm}p{6mm}p{7mm}|p{3.8mm}p{6mm}p{7mm}|p{3.8mm}p{6mm}p{7mm}|p{3.8mm}p{6mm}p{7mm}|p{3.8mm}p{6mm}p{7mm}|p{3.8mm}p{6mm}p{7mm}}\toprule
~ & \multicolumn{6}{c|}{\textbf{Index}} & \multicolumn{6}{c|}{\textbf{Middle}} & \multicolumn{6}{c}{\textbf{Ring}} \\ \cline{2-19}
\textbf{Prot-}&\multicolumn{3}{c|}{\textbf{Dev Set}} & \multicolumn{3}{c|}{\textbf{Eval Set}}&\multicolumn{3}{c|}{\textbf{Dev Set}} & \multicolumn{3}{c|}{\textbf{Eval Set}}&\multicolumn{3}{c|}{\textbf{Dev Set}} & \multicolumn{3}{c}{\textbf{Eval Set}}\\
\textbf{ocol} & \textbf{FMR} & \textbf{FNMR} & \textbf{HTER} & \textbf{FMR} & \textbf{FNMR} & \textbf{HTER} & \textbf{FMR} & \textbf{FNMR} & \textbf{HTER} & \textbf{FMR} & \textbf{FNMR} & \textbf{HTER} & \textbf{FMR} & \textbf{FNMR} & \textbf{HTER} & \textbf{FMR} & \textbf{FNMR} & \textbf{HTER} \\ \hline
P1  & 0.1  & 4.17 & 2.13  & 0.31 & 8.73  & 4.52 & 0.1  & 4.02 & 2.06 & 0.05 & 9.03  & 4.54 & 0.1  & 3.57 & 1.83 & 0.0 & 4.44 & 2.22 \\
P2  & 0.08 & 8.86 & 4.47  & 0.0  & 10.27 & 5.14 & 0.08 & 6.76 & 3.42 & 0.0  & 11.16 & 5.58 & 0.08 & 4.2 & 2.14  & 0.09  & 4.46 & 2.28 \\
P3 & 0.05  & 6.93 & 3.49  & 0.0  & 5.75  & 2.87 & 0.05 & 4.52 & 2.28 & 0.10 & 8.32  & 4.21 & 0.05 & 3.61 & 1.83 & 0.0  & 4.84  & 2.42 \\
P4 & 0.06  & 9.64 & 4.85  & 0.0  & 10.87 & 5.44 & 0.06 & 4.64 & 2.35 & 0.06 & 5.70  & 2.88 & 0.06 & 3.04 & 1.55 & 0.0  & 5.17 & 2.58 \\
%
P5  & 0.06 & 0.17 & 0.11 & 0.81 & 1.99   & 1.4  & 0.06 & 0.16 & 0.85 & 0.29 & 0.17  & 0.23 & 0.06 & 0.16 & 0.11 & 0.0 & 0.0  &\textbf{0.0} \\
P6  & 0.07 & 0.0  & 0.03 & 0.45 & 1.81  & \textbf{1.13} & 0.07 & 0.0  & 0.03 & 0.90 & 0.0  & 0.45 & 0.07 & 2.07 & 1.07 & 0.0 & 0.0  & \textbf{0.0} \\
P7 & 0.06 & 0.84 & 0.45  & 1.25 & 1.02 & 1.14   & 0.06 & 0.17 & 0.11 & 0.0 & 0.34  & \textbf{0.17} & 0.06 & 0.0  & 0.03 & 0.0 & 0.0  & \textbf{0.0} \\
P8 & 0.08 & 2.55 & 1.32  & 0.0  & 2.78  & 1.39  & 0.08 & 0.46 & 0.27 & 0.0  & 2.78  & 1.39 & 0.08 & 1.16 & 0.62 & 0.0  & 1.51 & 0.76 \\ \bottomrule
\end{tabular}
\label{tab:each_fing_rec_far0.1}
\vspace{-3mm}
\end{table*}

%% 
%\begin{table*}
%\caption{\small Middle-Finger-vein recognition performance at at FMR no greater than 0.1\% on the Dev set. 
%%HTER is the average of the FMR and the FNMR in each row.
%%The FMR, FNMR and HTER values in the table indicate percentages.
%%The score-threshold has been computed to achieve the desired FMR (0.1\%) on the Dev set. This score-threshold has then been applied to the comparison-scores obtained from the Eval set.
%The lowest HTER for this finger is marked in bold characters, and comes from RH\_right\_850 protocol.}
%\ra{1.1}
%\center
%\vspace{-3mm}
%\begin{tabular}{l|rrr|rrr|rrr|rrr}\toprule
%~ & \multicolumn{6}{c|}{\textbf{Index}} & \multicolumn{6}{c|}{\textbf{Middle}} \\
%\textbf{Protocol}&\multicolumn{3}{c|}{\textbf{Dev Set}} & \multicolumn{3}{c}{\textbf{Eval Set}}&\multicolumn{3}{c|}{\textbf{Dev Set}} & \multicolumn{3}{c}{\textbf{Eval Set}}\\
%~ & \textbf{FMR} & \textbf{FNMR} & \textbf{HTER} & \textbf{FMR} & \textbf{FNMR} & \textbf{HTER} & \textbf{FMR} & \textbf{FNMR} & \textbf{HTER} & \textbf{FMR} & \textbf{FNMR} & \textbf{HTER} \\ \hline
%P1 & 0.1  & 4.02 & 2.06 & 0.05 & 9.03 & 4.54 \\
%P2 & 0.08 & 6.76 & 3.42 & 0.0  & 11.16 & 5.58 \\
%P3 & 0.05 & 4.52 & 2.28 & 0.10  & 8.32  & 4.21 \\
%P4 & 0.06 & 4.64 & 2.35 & 0.06  & 5.70 & 2.88 \\
%%
%P5 & 0.06 & 0.16 & 0.85 & 0.29 & 0.17  & 0.23 \\
%P6 & 0.07 & 0.0  & 0.03 & 0.90 & 0.0  & 0.45 \\
%P7 & 0.06 & 0.17 & 0.11 & 0.0 & 0.34  & \textbf{0.17} \\
%P8 & 0.08 & 0.46 & 0.27 & 0.0  & 2.78  & 1.39 \\ \bottomrule
%\end{tabular}
%\label{tab:all_fing_rec_far0.1}
%%\vspace{-3mm}
%\end{table*}

%% this table is correct
%\begin{table}[H]
%\caption{\small Ring-Finger-vein recognition performance at FMR no greater than 0.1\% on the Dev set. 
%%HTER for each set is the average of the FMR and the FNMR in each row.
%%The FMR, FNMR and HTER values in the table indicate percentages.
%%The score-threshold has been computed to achieve the desired FMR (0.1\%) on the Dev set. This score-threshold has then been applied to the comparison-scores obtained from the Eval set.
%The lowest HTER for this finger are marked in bold characters, and come from three right-hand protocols.
%}
%\ra{1.1}
%\center
%\vspace{-3mm}
%\begin{tabular}{l|rrr|rrr}\toprule
%\textbf{Protocol}&\multicolumn{3}{c|}{\textbf{Dev Set}} & \multicolumn{3}{c}{\textbf{Eval Set}}\\
%~ & \textbf{FMR} & \textbf{FNMR} & \textbf{HTER} 
%%& \textbf{Threshold} 
%& \textbf{FMR} & \textbf{FNMR} & \textbf{HTER} \\ \hline
%P1 & 0.1  & 3.57 & 1.83 & 0.0 & 4.44 & 2.22 \\
%P2 & 0.08 & 4.2 & 2.14  & 0.09  & 4.46 & 2.28 \\
%P3 & 0.05 & 3.61 & 1.83 & 0.0  & 4.84  & 2.42 \\
%P4 & 0.06 & 3.04 & 1.55 & 0.0  & 5.17 & 2.58 \\
%%
%P5 & 0.06 & 0.16 & 0.11 & 0.0 & 0.0  &\textbf{ 0.0} \\
%P6 & 0.07 & 2.07 & 1.07 & 0.0 & 0.0  & \textbf{0.0} \\
%P7 & 0.06 & 0.0  & 0.03 & 0.0 & 0.0  & \textbf{0.0} \\
%P8 & 0.08 & 1.16 & 0.62 & 0.0  & 1.51 & 0.76 \\ \bottomrule
%\end{tabular}
%\label{tab:ring_fing_rec_far0.1}
%\vspace{-3mm}
%\end{table}
%%

